Challenging but Full of Opportunities: Teachers' Perspectives on Programming in Primary Schools

The widespread establishment of computational thinking in school curricula requires teachers to introduce children to programming already at primary school level. As this is a recent development, primary school teachers may neither be adequately prepared for how to best teach programming, nor may they be fully aware why they have to do so. In order to gain a better understanding of these questions, we contrast insights taken from practical experiences with the anticipations of teachers in training. By surveying 200 teachers who have taught programming at primary schools and 97 teachers in training, we identify relevant challenges when teaching programming, opportunities that arise when children learn programming, and strategies how to address both of these in practice. While many challenges and opportunities are correctly anticipated, we find several disagreements that can inform revisions of the curricula in teaching studies to better prepare primary school teachers for teaching programming at primary schools.

==> tables/challAnalysisTools.tex <==
\begin{table}[t]\centering
	\caption{Explanation of opinions on analysis tools by \tpEnd. \\
	%\textmd{The percentage corresponds to the proportion of \tp mentioning the category at least once.}
	}
	\label{tab:challsAnalysisToolsCodingScheme}
	\setlength{\tabcolsep}{0.2em}
	%\resizebox{\columnwidth}{!}{
\begin{tabular}{lrlp{4.7cm}}
	\toprule
	Category & \% TP & \hspace{\MAX} & Subcategories (\% TP) 
	\\
	\midrule
	
	Target group & \printpercent{\StrategyPercentAnalysisToolstargetgroup} & \DrawPercentageBar{\StrategyPercentAnalysisToolstargetgroup} & for teachers% (\printpercent{\StrategyPercentAnalysisToolstargetgroupforteachers})
	, general usefulness%  (\printpercent{\StrategyPercentAnalysisToolstargetgroupgeneralusefulness})
	, for students% (\printpercent{\StrategyPercentAnalysisToolstargetgroupforstudents}) 
	\\
	
	
	Uncertainty & \printpercent{\StrategyPercentAnalysisToolsuncertainty} & \DrawPercentageBar{\StrategyPercentAnalysisToolsuncertainty} & no experience% (\printpercent{\StrategyPercentAnalysisToolsuncertaintynoexperience})
	, no understanding% (\printpercent{\StrategyPercentAnalysisToolsuncertaintynounderstanding}) 
	\\
	
	
	Use cases & \printpercent{\StrategyPercentAnalysisToolsusecases} & \DrawPercentageBar{\StrategyPercentAnalysisToolsusecases} & feedback%  (\printpercent{\StrategyPercentAnalysisToolsusecasesfeedback})
	, debugging% (\printpercent{\StrategyPercentAnalysisToolsusecasesdebugging})
	, diagnosis% (\printpercent{\StrategyPercentAnalysisToolsusecasesdiagnosis})
	, support and tendencies% (\printpercent{\StrategyPercentAnalysisToolsusecasessupportandtendencies})
	, assessment %(\printpercent{\StrategyPercentAnalysisToolsusecasesassessment}) 
	\\
	
	
	Advantages & \printpercent{\StrategyPercentAnalysisToolsadvantages} & \DrawPercentageBar{\StrategyPercentAnalysisToolsadvantages} & deal with many students at the same time% (\printpercent{\StrategyPercentAnalysisToolsadvantagesdealwithmanystudents})
	, independence from the teacher% (\printpercent{\StrategyPercentAnalysisToolsadvantagesindependenceoftheteacher})
	, easy% (\printpercent{\StrategyPercentAnalysisToolsadvantagesimmediate})
	, more confidence of teachers% (\printpercent{\StrategyPercentAnalysisToolsadvantagesmoreconfidenceofteachers})
	, continuous %(\printpercent{\StrategyPercentAnalysisToolsadvantagescontinuous}) 
	\\
	
	
	Aims & \printpercent{\StrategyPercentAnalysisToolsaims} & \DrawPercentageBar{\StrategyPercentAnalysisToolsaims} & time% (\printpercent{\StrategyPercentAnalysisToolsaimstime})
	, students' acquisition of competencies% (\printpercent{\StrategyPercentAnalysisToolsaimsstudentsacquisitionofcompetencies}) 
	\\
	
		
	Disadvantages & \printpercent{\StrategyPercentAnalysisToolsdisadvantages} & \DrawPercentageBar{\StrategyPercentAnalysisToolsdisadvantages} & insufficient% (\printpercent{\StrategyPercentAnalysisToolsdisadvantagesinsufficient})
	, task of the teacher% (\printpercent{\StrategyPercentAnalysisToolsdisadvantagestaskoftheteacher})
	, no individualisation% (\printpercent{\StrategyPercentAnalysisToolsdisadvantagesnoindividualisation})
	, complex%(\printpercent{\StrategyPercentAnalysisToolsdisadvantagescomplex}) 
	\\
	
	
	Alternatives & \printpercent{\StrategyPercentAnalysisToolsalternatives} & \DrawPercentageBar{\StrategyPercentAnalysisToolsalternatives} & human feedback% (\printpercent{\StrategyPercentAnalysisToolsalternativeshumanfeedback})
	, not only tools% (\printpercent{\StrategyPercentAnalysisToolsalternativesnotonlytools}) 
	\\
	

\bottomrule
\end{tabular}
%}
\end{table}

==> tables/challStrategies.tex <==
\begin{table*}[t]\centering
	\caption{Coding scheme for strategies to master challenges.} 
	\label{tab:challStrategiesCodingScheme}
	\vspace{-1em}
	\setlength{\tabcolsep}{0.2em}
	\resizebox{0.9\textwidth}{!}{
\begin{tabular}{llp{11cm}rl}
	\toprule
	Category & Subcategory & Themes & \% TP 
	\\
	\midrule
	\rowcolor{Gray}
	
	Teachers &  & &  \printpercent{\StrategyPercentStrategiesforChallengesTeachers}  & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesTeachers}  \\
	& training & more, feasibly embedded, better training, self study & \printpercent{\StrategyPercentStrategiesforChallengesTeachersparticipateintraining}  & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesTeachersparticipateintraining} \\
    & teaching & use different methods, simplify, consider individual factors, divide into groups, expand students' prior knowledge, increase engagement, teach interdisciplinary, plan ahead & \printpercent{\StrategyPercentStrategiesforChallengesTeachersteaching}  & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesTeachersteaching} \\
    & content of training & affective, content knowledge, pedagogical content knowledge, trying out & \printpercent{\StrategyPercentStrategiesforChallengesTeacherscontentoftraining} & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesTeacherscontentoftraining}  \\
    & cooperate & experts, teachers, additional helpers & \printpercent{\StrategyPercentStrategiesforChallengesTeacherscooperatewithothers}  & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesTeacherscooperatewithothers} \\
    & time & more often, slow, one dedicated time & \printpercent{\StrategyPercentStrategiesforChallengesTeacherstime}  & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesTeacherstime} \\
    & use material & schemes of work, programs & \printpercent{\StrategyPercentStrategiesforChallengesTeachersgetsupportthroughmaterial}  & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesTeachersgetsupportthroughmaterial} \\
	\rowcolor{Gray}
    
    
    School & & &  \printpercent{\StrategyPercentStrategiesforChallengesSchool} & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesSchool}    \\
     & media equipment & buy equipment, collect donations, request, prioritise, provide equipment for home, save money  & \printpercent{\StrategyPercentStrategiesforChallengesSchoolmediaequipment} & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesSchoolmediaequipment}  \\
    & course after school & &  \printpercent{\StrategyPercentStrategiesforChallengesSchoolcourseafterschool} & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesSchoolcourseafterschool}  \\
    & joint approach & &  \printpercent{\StrategyPercentStrategiesforChallengesSchooljointapproach} & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesSchooljointapproach}  \\
    & responsible teacher & &  \printpercent{\StrategyPercentStrategiesforChallengesSchoolresponsibleteacher} & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesSchoolresponsibleteacher}  \\
	\rowcolor{Gray}
	
	
	Government &  & &  \printpercent{\StrategyPercentStrategiesforChallengesGovernment} & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesGovernment}  \\
	 & more funds for CSE & &  \printpercent{\StrategyPercentStrategiesforChallengesGovernmentmorefundsforCSE} & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesGovernmentmorefundsforCSE} \\
	& reorganise curricula & more relevance, start earlier, start later & \printpercent{\StrategyPercentStrategiesforChallengesGovernmentreorganisecurricula} & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesGovernmentreorganisecurricula} \\
	\rowcolor{Gray}


	Parents & & &  \printpercent{\StrategyPercentStrategiesforChallengesParents}  & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesParents}   \\
	 & content & affective, general inclusion, cognitive & \printpercent{\StrategyPercentStrategiesforChallengesParentsContent}  & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesParentsContent} \\
	& meetings & &  \printpercent{\StrategyPercentStrategiesforChallengesParentsMeetings}  & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesParentsMeetings} \\
	& support & &  \printpercent{\StrategyPercentStrategiesforChallengesParentsMeetings}  & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesParentsMeetings} \\
	\rowcolor{Gray}
    
    
    Society & & & \printpercent{\StrategyPercentStrategiesforChallengesSociety}  & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesSociety} \\
     & rethink sociologically & & \printpercent{\StrategyPercentStrategiesforChallengesSocietyrethinksociologically}  & \DrawPercentageBar{\StrategyPercentStrategiesforChallengesSocietyrethinksociologically} \\
    
    

\bottomrule
\end{tabular}
}
\end{table*}

==> tables/oppStrategiesCodingScheme.tex <==
\begin{table*}[t]\centering
	\caption{Coding Scheme for Strategies for Opportunities.}
	\vspace{-1em}
	\label{tab:oppStrategiesCodingScheme}
	\resizebox{\textwidth}{!}{
\begin{tabular}{llp{10cm}}
	
\toprule
Area & Category & Statement \\ \midrule

Affective Factors & Improving affective factors &    \\
&  Change of mindset of parents and teachers, integration  & \\
&  Enthusiasm (role model) and encouragement of students  &   \\

Cross-curricular learning & &  \\

Early support &  & \\

Gaining (computer) skills &  &  \\

Inviting experts &  &\\

Methodical-didactical approach & Activities, courses, challenges, homework &  \\
 &  addressing individual needs, learning strategies, heterogeneity &  \\
 &  feedback &    \\
 &  programs &   \\
 &  teamwork &   \\

Requirements (e.g. equipment of schools, time in the curriculum, training of teachers) &  &    \\

Social and private importance & explaining the relevance of programming  &   \\
&  pointing out future (job) opportunities&   \\
&  product orientation&  \\
&  student's lifeworld&    \\
&  practical application& \\

Stimulating alternative ways of thinking  &  &  \\

Stimulating students' creativity  &  &   \\

Other &  &    \\

	
\bottomrule
\end{tabular}
}
\end{table*}
